Unsupervised Defect Detection for Surgical Instruments

Ensuring the safety of surgical instruments requires reliable detection of visual defects. However, manual inspection is prone to error, and existing automated defect detection methods, typically trained on natural/industrial images, fail to transfer effectively to the surgical domain. We demonstrate that simply applying or fine-tuning these approaches leads to issues: false positive detections arising from textured backgrounds, poor sensitivity to small, subtle defects, and inadequate capture of instrument-specific features due to domain shift. To address these challenges, we propose a versatile method that adapts unsupervised defect detection methods specifically for surgical instruments. By integrating background masking, a patch-based analysis strategy, and efficient domain adaptation, our method overcomes these limitations, enabling the reliable detection of fine-grained defects in surgical instrument imagery.

==> 2_related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Defect Detection}
Visual defect detection has become a central topic in industrial quality control, where detecting subtle defects is crucial for ensuring product reliability and safety. Methods in this field can be broadly categorized into embedding similarity-based approaches and reconstruction-based approaches. Embedding similarity-based methods, such as PatchCore~\cite{patchcore} and PaDiM~\cite{padim}, leverage pre-trained deep feature extractors to compute the similarity between input images and a database of normal patterns. These methods have achieved strong performance on industrial benchmarks like MVTec AD~\cite{mvtec}. Reconstruction-based methods attempt to learn the distribution of normal data by training models to reconstruct input images, identifying anomalies through discrepancies between the input and reconstruction. These approaches~\cite{liu2024deep, xie2024iad} can be supervised or unsupervised, with the latter trained exclusively on normal, defect-free data. In industrial practice, supervised reconstruction-based methods are limited by the scarcity of labeled defect data and the high cost of annotation. As a result, unsupervised methods, particularly those based on autoencoders~\cite{mvtec, liang2023omni}, have become increasingly attractive for scenarios where only normal data is readily available.

% \subsection{Domain Adaptation and Foundation Models}
% To handle domain shifts without the computational expense of training the models, recent studies rely on foundation models and efficient adaptation strategies. The Segment Anything Model (SAM) \cite{kirillov2023segment} has shown strong zero-shot performance for object isolation, which we utilize to remove background noise. In addition, Parameter-Efficient Fine-Tuning (PEFT) \cite{han2024parameter} approaches, particularly Low-Rank Adaptation (LoRA) \cite{hu2022lora}, enable large pre-trained encoders to be fine-tuned for particular downstream tasks by learning low-rank updates while holding the original weights fixed. This strategy has been shown to be effective for preserving general visual insights while capturing domain-specific subtleties, making it particularly suited for adapting natural image encoders to the geometries and textures of surgical tools.

